Early Work on Efficient Patching for Coordinating Edge Applications

Multiple applications running on Edge computers can be orchestrated to achieve the desired goal. Orchestration of applications is prominent when working with Internet of Things based applications, Autonomous driving and Autonomous Aerial vehicles. As the applications receive modified classifiers/code, there will be multiple applications that need to be updated. If all the classifiers are synchronously updated there would be increased throughput and bandwidth degradation. On the other hand, delaying updates of applications which need immediate update hinders performance and delays progress towards end goal. The updates of applications should be prioritized and updates should happen according to this priority. This paper explores the setup and benchmarks to understand the impact of updates when multiple applications working to achieve same objective are orchestrated with prioritized updates. We discuss methods to build a distributed, reliable and scalable system called "DSOC"(Docker Swarm Orchestration Component).

==> algorithms/algorithm.tex <==
% This is from what Naveen has understood and thought about in mind.
\textbf{Pre-conditions:} A Docker containerized Application which uses field data and ML model for decision making. "Chimera Engine" which continuously tracks Application and make sure Autonomy criteria is satisfied. "Cloudlet" segregates and fragments the application components. It computes efficient model to be chosen.

AC = Autonomy Criteria, like Energy, Accuracy, latency and storage.
ACC = Accuracy
E = Energy
S = Storage
L = Latency

At the source/edge computer: while (AC ! satisfied)
{
1.Chimera Engine tracks the new AC requirements
2.Cloudlet uses Best Model Chooser Algorithm to find 3-5 best models and dumps them to a priority\_queue.
3. Only diff of updated model and original model is tracked by Chimera Engine. This is sent back to edge computer and model is updated.
}

==> algorithms/tput_accuracy_algorithm.tex <==
%% From Chris's idea, if multiple models need to be updated synchronously there will be huge degradation of throughput.


%%% SO how do we decide between accuracy and tput factors in a rich workload system..??

% As application scales, there would be multiple models, multiple AC. How do we decide and balance which model to update and which model to halt???

==> bibliographybibnaveen.tex <==

\bibitem{c1} C. Katrakazas, M. Quddus, W.H. Chen, L. Deka, "Real-time motion planning methods for autonomous on-road driving: State-of-the-art and future research directions" Transportation Research Part C: Emerging Technologies, Volume 60, pp. 416-442, 2015. 

\bibitem{c2} L. K. A. Levy, "Self-driving cars take over CES: Here's how big tech is playing the market," CNBC, 12 Jan 2018. [Online]. Available: https://www.cnbc.com/2018/01/12/intel-cisco-and-amazon-introduce-self-driving-car-technology-at-ces.html. [Accessed 15 Jan 2019].
\bibitem{c3} A. Choudhary, M.C. Govil, G. Singh, L.K Ashwathi, E.S. Pilli, D. Kapil, "A critical survey of live virtual machine migration techniques," Journal of Cloud ComputingAdvances, Systems and Applications, vol. 6, pp. 1-41, 2017.
\bibitem{c4} M. I. Jordan, T. M. Mitchell, "Machine learning: Trends, perspectives, and prospects," Science, vol. 349, no. 6245, pp. 255-260, 2015.
\bibitem{c5} Docker Inc., "What is a container," Docker Inc, 2018. [Online]. Available: https://www.docker.com/resources/what-container. [Accessed 15 Jan 2019].
\bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
\bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
\bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
\bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 









==> coalescer.tex <==
\section{Coalescer and Stratagem Functionality}

 %The Coalescer component, consisting of manager nodes, has three main functionalities:

%\begin{enumerate}
%   \item Track the changes in applications and report them to Strategem.
%    \item It handles the migration of model or data from Stratagem to Application or vice-versa.
%    \item It also makes sure that system specified autonomy criteria is being satisfied. It aggregates each application's performance and aggregated them to make sure overall system specified performance criteria is being satisfied.
%\end{enumerate}
%The Strategem component, consisting of worker nodes, has three main functionalities:
%\begin{enumerate}
%    \item Record the per-application contents and update further changes to the application.
%    \item Maintain a list of best models. Newer models can be generated based on updates to autonomy criteria. A newer model of less size, greater accuracy, lesser energy can be generated and later used by the application.
%    \item Whenever the current model 'm\_curr' need to be updated with a better model 'm\_betr', the diff of m\_curr and m\_betr would be transferred from Stratagem to Application with the help of Coalescer.
%\end{enumerate}






==> implement_orig.tex <==
\MYnote{
\begin{algorithm}
\caption{Greedy Method}
\begin{algorithmic}[1]
\State $\textit{update\_queue = {initialize with set of Model_{ij}}}$
\While{$\textit{update\_queue is not empty}$}
\IF{$\textit{updated Model_ij is available}$}
\State $\textit{update_queue = {Append all updated Model_ij}}$
\EndIf
\IF{$\textit{System specific parameters look fine}$}
\State $\textit{Choose 'K' models for synchronous update}$
\State $\textit{Assign worker_i to update Model_ij}$
\EndIf
\ELSE 
\State $\textit{Delay update task till system performance improves}$
\EndElse
\EndWhile
\end{algorithmic}
\end{algorithm}
}


second onee


\begin{algorithm}
\caption{DSOC method}
\begin{algorithmic}[2]
\State $\textit{update\_queue = {initialize with set of Model_{ij}}}$
\While{$\textit{update\_queue is not empty}$}
\IF{$\textit{updated Model_ij is available}$}
\State $\textit{update_queue = {Append all updated Model_ij}}$
\EndIf

\State $\textit{assign_priority(M, system params, Application params}$
\end{algorithmic}
\end{algorithm}


%%%% Main calculation equation

% Function assign_priority()
\begin{algorithm}
 \caption{Prioritizing application update}
  \begin{algorithmic}[1]
   \Function{Assign Priority}{sParams,sWeights,aParams,aWeights}  % try to work on these terminologies...
   %\State $\text{System_Perf_value = a1 * (c_ij/(c_free + c_i)) + a2 * (m_ij/(m_free + m_i)) + a3 * (s_ij/(s_free + s_i)) + a4 * (t_ij/ sum(ti)) }$
   
   % Need to write a similar Equation for applicatio specific parameters also. Look at the equation below...
   
   %\State $\text{ Applic_Perf_value = b1 * (acc_ij-paccij/(accij + paccij)/2) + b2 * (pr_ij-Eprij/(prij + Eprij)/2) + b3 * (lat/Elatij) + b4 * (execution_time/avg execution time of apps in that node)}$
   
   
   
   % cpu util/total cpu ---fine
   % memory-used/total memeory --fine
   % storage used/total storage
   % Bandwidthj/# of containers > thresholdBandwidth
   % tput within node, tputij = tpt/sumof all tputj -- To make sure all apps within a node get fair chance to update their model.
   %\State 
   
   %\State $\text{System_Perf_value = sum of all i Sp_val * weight of that feature}$
   %\State $\text{Application_Perf_value = sum of all i App_val * weight of that feature}$
   % \State $\textit{Overall_Perf_value = alpha * System_Perf + Beta * Application_Perf}$
   \State $\textit{priority} \gets \text\{{Green, Yellow, Blue, Red}\}$
   \EndFunction




\end{algorithmic}
\end{algorithm}


